Are Bias Mitigation Techniques for Deep Learning Effective?

A critical problem in deep learning is that systems learn inappropriate biases, resulting in their inability to perform well on minority groups. This has led to the creation of multiple algorithms that endeavor to mitigate bias. However, it is not clear how effective these methods are. This is because study protocols differ among papers, systems are tested on datasets that fail to test many forms of bias, and systems have access to hidden knowledge or are tuned specifically to the test set. To address this, we introduce an improved evaluation protocol, sensible metrics, and a new dataset, which enables us to ask and answer critical questions about bias mitigation algorithms. We evaluate seven state-of-the-art algorithms using the same network architecture and hyperparameter selection policy across three benchmark datasets. We introduce a new dataset called Biased MNIST that enables assessment of robustness to multiple bias sources. We use Biased MNIST and a visual question answering (VQA) benchmark to assess robustness to hidden biases. Rather than only tuning to the test set distribution, we study robustness across different tuning distributions, which is critical because for many applications the test distribution may not be known during development. We find that algorithms exploit hidden biases, are unable to scale to multiple forms of bias, and are highly sensitive to the choice of tuning set. Based on our findings, we implore the community to adopt more rigorous assessment of future bias mitigation methods. All data, code, and results are publicly available at: https://github.com/erobic/bias-mitigators.

==> tables/biased-mnist-bkg-color-results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Biased MNIST Accuracies, using background color as the explicit bias variable for all methods except Base, LFF and SD.}
\label{tbl:biased_mnist_results_bkg_color}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllllllllll}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Bias Variables/\\ Methods\end{tabular}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Balanced\\ Test\end{tabular}}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Background \\ Color\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Digit \\ Color\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Digit \\ Position\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Distractor\\ Shape\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Distractor \\ Color\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{Texture}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Texture\\ Color\end{tabular}}} \\
\textbf{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textbf{Maj.}} &
  \multicolumn{1}{c}{\textbf{Min.}} &
  \multicolumn{1}{c}{\textbf{Maj.}} &
  \multicolumn{1}{c}{\textbf{Min.}} &
  \multicolumn{1}{c}{\textbf{Maj.}} &
  \multicolumn{1}{c}{\textbf{Min.}} &
  \multicolumn{1}{c}{\textbf{Maj.}} &
  \multicolumn{1}{c}{\textbf{Min.}} &
  \multicolumn{1}{c}{\textbf{Maj.}} &
  \multicolumn{1}{c}{\textbf{Min.}} &
  \multicolumn{1}{c}{\textbf{Maj.}} &
  \multicolumn{1}{c}{\textbf{Min.}} &
  \multicolumn{1}{c}{\textbf{Maj.}} &
  \multicolumn{1}{c}{\textbf{Min.}} \\\hline
\textbf{conventional}  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{Up Wt} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{GDRO}  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{RUBi}  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{LNL}   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{IRMv1} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{LFF}   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{SD}    &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}%
}
\end{table*}

==> tables/biased-mnist-expl-impl.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Biased MNIST Accuracies based on explicit and implicit variables.}
\label{tbl:biased_mnist_expl_impl}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{llll|lll} \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Bias Type/\\ Methods\end{tabular}} &
  \multicolumn{3}{c}{Explicit} &
  \multicolumn{3}{c}{Implicit} \\
 &
  \multicolumn{1}{c}{MPG} &
  \multicolumn{1}{c}{Maj.} &
  \multicolumn{1}{c}{Min.} &
  \multicolumn{1}{c}{MPG} &
  \multicolumn{1}{c}{Maj.} &
  \multicolumn{1}{c}{Min.} \\ \hline
\gls*{conventional}  & N/A & N/A  &  N/A & ? & ? & ? \\
Up Wt~\cite{sagawa2020investigation} & ? & ? & ? & ? & ? & ? \\
GDRO~\cite{sagawa2019distributionally}  &  &  &  &  &  &  \\
RUBi~\cite{cadene2019rubi}  &  &  &  &  &  &  \\
LNL~\cite{kim2019learning}   &  &  &  &  &  &  \\
IRMv1~\cite{arjovsky2019invariant} &  &  &  &  &  &  \\
LFF~\cite{nam2020learning}   &  &  &  &  &  &  \\
SD~\cite{pezeshki2020gradient}    &  &  &  &  &  & \\ \hline
\end{tabular}%
}
\end{table}

==> tables/biased-mnist-increasing-explicit-biases.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Accuracy as new bias variables are added to explicit methods. Base, LFF and SD are invariant to the choice of explicit bias during training.}
\label{tbl:biased_mnist_increasing_explicit_biases}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc} \hline
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Explicit\\ Variables/\\ Methods\end{tabular}} &
  Distractor Shape &
  +Texture &
  \begin{tabular}[c]{@{}c@{}}+Digit \\ Color\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}+Background\\ Color\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}+Texture\\ Color\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}+Distractor\\ Color\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}+Digit\\ Position\end{tabular} \\ \hline
\gls*{conventional}  & \multicolumn{7}{c}{---------------------------------- 50.3 ----------------------------------} \\
Up Wt & 23.2        & 15.7        & 14.1        & 31.4        & 41.5         & 49.2       & 47.6       \\
GDRO  & 25.4        & 19.0        & 19.1        & 20.9        & 21.5         & 20.2       & 17.0       \\
RUBi  & 31.9        & 32.8        & 10.8        & 9.8         & 9.8          & 10.0       & 10.2       \\
LNL   & 63.8        & 10.0        & 10.0        & 10.0        & 10.0         & 10.0       & 10.0       \\
IRMv1 & 46.5        & 40.7        & 24.3        & 24.3        & 31.0        & 24.8       & 21.7       \\
LFF   & \multicolumn{7}{c}{---------------------------------- 63.2 ----------------------------------} \\
SD    & \multicolumn{7}{c}{---------------------------------- 45.2 ----------------------------------} \\ \hline
\end{tabular}%
%}
\end{table*}

==> tables/celebA-results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{CelebA accuracies.}
\label{tbl:celebA-results}
\begin{tabular}{l|rr|rr|r|r}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Groups/\\ Methods\end{tabular}}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Blond Hair \\ Color\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Non-Blond\\ Hair Color\end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Unbiased \\ Accuracy\end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Overall\\ Accuracy\end{tabular}}} \\ \hline
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\textbf{Male}} &
  \multicolumn{1}{c}{\textbf{Female}} &
  \multicolumn{1}{c}{\textbf{Male}} &
  \multicolumn{1}{c}{\textbf{Female}} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\ \hline
\gls*{conventional}  & 30.7 & 79.1 & 99.0 & 95.9 & 76.2 &  \\
Up Wt &      &      &      &      &      &  \\
GDRO  &      &      &      &      &      &  \\
RUBi  &      &      &      &      &      &  \\
LNL   &      &      &      &      &      &  \\
IRMv1 &      &      &      &      &      &  \\
LFF   &      &      &      &      &      &  \\
SD    &      &      &      &      &      & \\
\hline
\end{tabular}%
\end{table}

==> tables/gqa-expl-bias-head-vs-tail.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{GQA head and tail accuracies considering different variables as explicit biases.}
\label{tbl:gqa_expl_bias_head_vs_tail}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{lll|lcccccccc} \hline
\begin{tabular}[c]{@{}l@{}}Implicit \\ Methods\end{tabular} &
   &
   &
  \begin{tabular}[c]{@{}l@{}}Explicit Variables/\\ Explicit Methods\end{tabular} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Head/Tail\\ (2 groups)\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Answer Class\\ (1833 groups)\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Global Group\\ (115 groups)\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Local Group\\ (133328 groups)\end{tabular}} \\ \hline
     & Head & Tail &       & Head & Tail & Head & Tail & Head & Tail & Head & Tail \\ \hline
\gls*{conventional} & 49.5 & 40.1 & Up Wt & 47.0 & 39.6 & 28.1 & 23.9 & 29.7 & 23.1 & 27.7 & 20.7 \\
LFF  & 37.5 & 36.5 & GDRO  & 51.4 & 42.5 & 33.5 & 23.6 & 13.6 & 7.9  & 21.6 & 17.2 \\
SD   & 48.8 & 45.0 & RUBi  & 46.6 & 41.6 & N/A  & N/A  & 5.8  & 5.5  & 25.0 & 20.2 \\
     &      &      & LNL   & 44.8 & 40.9 & N/A  & N/A  & 36.3 & 28.4 & 12.4 & 9.0  \\
     &      &      & IRMv1 & 49.4 & 45.0 & 39.0 & 32.6 & 41.5 & 39.3 & 35.9 & 31.7 \\ \hline
\end{tabular}%
%}
\end{table*}
